Coverage-based Scene Fuzzing for Virtual Autonomous Driving Testing

Simulation-based virtual testing has become an essential step to ensure the safety of autonomous driving systems. Testers need to handcraft the virtual driving scenes and configure various environmental settings like surrounding traffic, weather conditions, etc. Due to the huge amount of configuration possibilities, the human efforts are subject to the inefficiency in detecting flaws in industry-class autonomous driving system. This paper proposes a coverage-driven fuzzing technique to automatically generate diverse configuration parameters to form new driving scenes. Experimental results show that our fuzzing method can significantly reduce the cost in deriving new risky scenes from the initial setup designed by testers. We expect automated fuzzing will become a common practice in virtual testing for autonomous driving systems.

==> discussion.tex <==
AI Safety needs to be quantified through metrics to be compared with each other or with human performance.  However, self-driving companies submit on-road testing results voluntarily. The transparency and publicity of the information are questionable. And the coverage of unforeseen safety corner cases is limited. 

Analogous to our previous work~\cite{zhenyu.dsn.2020}, we believe the robustness metric also fits in the self-driving scenario. We believe it will be an aggregated robustness from its sub-components. For example, we have perception robustness, planning robustness, as well as fusion robustness. Uniquely, self-driving robustness depends on a sequence of events or consecutive frames for various sub-components instead of the DNN model robustness measured on perturbations to a single input image. Conceptually, we can define robustness based on the safety fuzzing results. Each discovered safety violation corresponds to a sequence of events. By replaying the driving scene with perturbations on the input sequence, we derive a legitimate sequence of events resulting in no violation. The robustness can be measured as the distance between the normal sequences and those that trigger the violation.
